QUIC Steps: Evaluating Pacing Strategies in QUIC Implementations

Pacing is a key mechanism in modern transport protocols, used to regulate packet transmission timing to minimize traffic burstiness, lower latency, and reduce packet loss. Standardized in 2021, QUIC is a UDP-based protocol designed to improve upon the TCP / TLS stack. While the QUIC protocol recommends pacing, and congestion control algorithms like BBR rely on it, the user-space nature of QUIC introduces unique challenges. These challenges include coarse-grained timers, system call overhead, and OS scheduling delays, all of which complicate precise packet pacing. This paper investigates how pacing is implemented differently across QUIC stacks, including quiche, picoquic, and ngtcp2, and evaluates the impact of system-level features like GSO and Linux qdiscs on pacing. Using a custom measurement framework and a passive optical fiber tap, we establish a baseline with default settings and systematically explore the effects of qdiscs, hardware offloading using the ETF qdisc, and GSO on pacing precision and network performance. We also extend and evaluate a kernel patch to enable pacing of individual packets within GSO buffers, combining batching efficiency with precise pacing. Kernel-assisted and purely user-space pacing approaches are compared. We show that pacing with only user-space timers can work well, as demonstrated by picoquic with BBR. With quiche, we identify FQ as a qdisc well-suited for pacing QUIC traffic, as it is relatively easy to use and offers precise pacing based on packet timestamps. Our findings provide new insights into the trade-offs involved in implementing pacing in QUIC and highlight potential optimizations for real-world applications like video streaming and video calls.

==> acronyms.tex <==
\DeclareAcronym{pt}{
    short               = {PT},
    long                = {Packet Train}
}

\DeclareAcronym{ptl}{
    short               = {PTL},
    long                = {Packet Train Length}
}

\DeclareAcronym{cpu}{
    short               = {CPU},
    long                = {CPU},
    first-style         = short,
}

\DeclareAcronym{ack}{
    short               = {ACK},
    long                = {acknowledgment},
}

\DeclareAcronym{aes}{
    short               = {AES},
    long                = {Advanced Encryption Standard},
}

\DeclareAcronym{chacha20}{
    short               = {ChaCha20},
    long                = {ChaCha20},
    first-style         = short,
}

\DeclareAcronym{qir}{
	short				= {QIR},
	long				= {QUIC Interop Runner},
}

\DeclareAcronym{io}{
    short               = {I/O},
    long                = {I/O},
    first-style         = short,
}

\DeclareAcronym{udp}{
	short				= {UDP},
	long				= {UDP},
	first-style			= short,
}

\DeclareAcronym{tcp}{
    short               = {TCP},
    long                = {TCP},
    first-style         = short,
}

\DeclareAcronym{tls}{
    short               = {TLS},
    long                = {Transport Layer Security},
    first-style         = short,
}

\DeclareAcronym{ietf}{
    short               = {IETF},
    long                = {Internet Engineering Task Force},
}

\DeclareAcronym{http}{
    short               = {HTTP},
    long                = {Hypertext Transfer Protocol},
    first-style         = short,
}

\DeclareAcronym{https}{
    short               = {HTTPS},
    long                = {Hypertext Transfer Protocol Secure},
    first-style         = short,
}

\DeclareAcronym{nic}{
    short               = {NIC},
    long                = {Network Interface Card},
}

\DeclareAcronym{tso}{
    short               = {TSO},
    long                = {TCP Segmentation Offload},
}

\DeclareAcronym{lro}{
    short               = {LRO},
    long                = {Large Receive Offload},
}

\DeclareAcronym{gso}{
    short               = {GSO},
    long                = {Generic Segmentation Offload},
}

\DeclareAcronym{gro}{
    short               = {GRO},
    long                = {Generic Receive Offload},
}

\DeclareAcronym{mss}{
    short               = {MSS},
    long                = {Maximum Segment Size},
}

\DeclareAcronym{rcvbuf}{
    short               = {RCVBUF},
    long                = {Receive Buffer},
}

\DeclareAcronym{sndbuf}{
    short               = {SNDBUF},
    long                = {Send Buffer},
}

\DeclareAcronym{cc}{
    short               = {CC},
    long                = {Congestion Control},
}

\DeclareAcronym{cca}{
    short               = {CCA},
    long                = {Congestion Control Algorithm},
}

\DeclareAcronym{bbr}{
    short               = {BBR},
    long                = {Bottleneck Bandwidth and RTT},
}

\DeclareAcronym{bdp}{
    short               = {BDP},
    long                = {Bandwidth-Delay Product},
}

\DeclareAcronym{os}{
    short               = {OS},
    long                = {Operating System},
}

\DeclareAcronym{tsn}{
    short               = {TSN},
    long                = {Time-Sensitive Networking},
}

\DeclareAcronym{qdisc}{
    short               = {qdisc},
    long                = {queueing discipline},
}

\DeclareAcronym{fq}{
    short               = {FQ},
    long                = {Fair Queue},
}

\DeclareAcronym{etf}{
    short               = {ETF},
    long                = {Earliest TxTime First},
}

\DeclareAcronym{fqcodel}{
    short               = {FQ\_CoDel},
    long                = {Fair Queuing Controlled Delay},
}

\DeclareAcronym{codel}{
    short               = {CoDel},
    long                = {Controlled Delay},
}

\DeclareAcronym{tbf}{
    short               = {TBF},
    long                = {Token Bucket Filter},
}

\DeclareAcronym{rtt}{
    short               = {RTT},
    long                = {Round-Trip Time},
}

\DeclareAcronym{cdf}{
    short               = {CDF},
    long                = {Cumulative Distribution Function},
}

